Architectural Support for Efficient Data Movement in Disaggregated Systems

Resource disaggregation offers a cost effective solution to resource scaling, utilization, and failure-handling in data centers by physically separating hardware devices in a server. Servers are architected as pools of processor, memory, and storage devices, organized as independent failure-isolated components interconnected by a high-bandwidth network. A critical challenge, however, is the high performance penalty of accessing data from a remote memory module over the network. Addressing this challenge is difficult as disaggregated systems have high runtime variability in network latencies/bandwidth, and page migration can significantly delay critical path cache line accesses in other pages. This paper introduces DaeMon, the first software-transparent and robust mechanism to significantly alleviate data movement overheads in fully disaggregated systems. First, to enable scalability to multiple hardware components in the system, we enhance each compute and memory unit with specialized engines that transparently handle data migrations. Second, to achieve high performance and provide robustness across various network, architecture and application characteristics, we implement a synergistic approach of bandwidth partitioning, link compression, decoupled data movement of multiple granularities, and adaptive granularity selection in data movements. We evaluate DaeMon in a wide variety of workloads at different network and architecture configurations using a state-of-the-art accurate simulator and demonstrate that DaeMon significantly improves system performance and data access costs over the widely-adopted approach of moving data at page granularity.

==> [HMC 2023] - DaeMon - 2-page Abstract/extended_abstract.tex <==

\section{Data Movement in Disaggregated Systems}
%\noindent\textbf{\large{1. Data Movement in Disaggregated Systems}}

\vspace{-2pt}
Traditional data centers include monolithic servers that tightly integrate CPU, memory and disk (Figure~\ref{fig:baseline-architecture-exab}a). Instead, \emph{Disaggregated Systems} (\textbf{\disaggrSystems{}})~\cite{Shan2018LegoOS,guo2021clio,Lee2021MIND} organize multiple compute (\textbf{\computeComponent{}}), memory (\textbf{\memoryComponent{}}) and storage devices as \emph{independent, failure-isolated} components interconnected over a high-bandwidth network (Figure~\ref{fig:baseline-architecture-exab}b). 
%, and thus can greatly reduce data center costs~\cite{Calciu2021Rethinking,Shan2018LegoOS}.
\disaggrSystems{} can greatly reduce data center costs by providing improved resource utilization, resource scaling, failure-handling and elasticity in modern data centers~\cite{Calciu2021Rethinking,Shan2018LegoOS,guo2021clio,Lee2021MIND,Giannoula2022Thesis}. \blfootnote{\textbf{* Kailong Huang and Jonathan Tang have equal contribution.}}


\begin{figure}[h]
    \vspace{-8pt}
    \centering
    \includegraphics[width=0.92\linewidth]{Baseline_Disaggr_System_ExAb.pdf}
    \vspace{-4pt}
    \caption{(a) Traditional systems vs (b) \disaggrSystems{}.}
    \label{fig:baseline-architecture-exab}
    \vspace{-7pt}
\end{figure}


The \memoryComponents{} provide large pools of main memory (\textbf{\emph{remote memory}}), while the \computeComponents{} include the on-chip caches and a few GBs of DRAM (\textbf{\emph{local memory}}) that acts as a cache of \emph{remote memory}.  In this context, a large fraction of the application's data ($\sim80$\%)~\cite{Shan2018LegoOS,Lee2021MIND,Gao2016Network} is located in \textit{remote memory}, and can cause large performance penalties (see Figure~\ref{fig:motivation-exab}) from remotely accessing data over the network.




Alleviating data access overheads is challenging in \disaggrSystems{} for the following reasons. First, \disaggrSystems{} are not monolithic and comprise independently managed entities: each component has its own hardware controller, and a specialized
kernel monitor uses its own functionality to manage the component it runs on (only communicates with other monitors via network messaging if there is a need to access remote
resources). This characteristic necessitates a distributed and disaggregated solution that can scale to a large number of independent components in the system. Second, there is high variability in remote memory access latencies since they depend on the locations of the \memoryComponents{}, contention from other jobs that share the same network and \memoryComponents{}, and data placements that can vary during runtime or between multiple executions. This necessitates a solution that is robust towards fluctuations in the network/remote memory bandwidth and latencies. Third, a major factor behind the performance slowdowns is the commonly-used approach in \disaggrSystems{}~\cite{Lee2021MIND,Shan2018LegoOS,Calciu2021Rethinking,Gao2016Network} of moving data at page granularity. This approach effectively provides software transparency, low metadata costs in memory management, and high spatial locality in many applications. However, it can cause high bandwidth consumption and network congestion, and often significantly slows down accesses to critical path cache lines in other concurrently accessed pages. 

%the coarse granularity at which data is typically moved in data centers~\cite{Lee2021MIND,Shan2018LegoOS,Calciu2021Rethinking,Gao2016Network}: migrating data at a page granularity (e.g., 4KB) provides software transparency, low metadata costs in memory management, and high spatial locality in many applications, however it can incur high bandwidth consumption and network congestion and/or significantly slow down accesses to cache lines in other concurrently accessed pages. 




Figure~\ref{fig:motivation-exab} presents a performance analysis of different data movement schemes using \disaggrSystems{} for a representative set of heterogeneous workloads. We evaluate a \memoryComponent{} and a \computeComponent{} with \emph{local memory} to fit $\sim$20\% of the application data, and the network bandwidth to be 1/2-1/8$\times$ of the bus bandwidth~\cite{Shan2018LegoOS,Gao2016Network}. Performance of all schemes is normalized to that of the monolithic approach where \emph{all} data fits in the \emph{local memory} of the \computeComponent{}. We make three observations.



\begin{figure}[h]
    \vspace{-6pt}
    \centering
    \includegraphics[width=\linewidth]{motivation_exab2_netlat_100_bwsf_2_ipc_slowdown.pdf}
    \includegraphics[width=\linewidth]{motivation_exab2_netlat_100_bwsf_8_ipc_slowdown.pdf}
    \vspace{-16pt}
    \caption{Data movement overheads in \disaggrSystems{}.}
    \label{fig:motivation-exab}
    \vspace{-8pt}
\end{figure}


First, the typically-used \emph{page} scheme of moving data at a page granularity incurs large slowdowns %(by 4.58$\times$) 
over the monolithic \emph{Local} configuration due to transferring large amounts of data over the network that slows down accesses to other pages. Instead, when pages are moved \revised{\emph{for free}}, i.e., \emph{page-free}, performance significantly improves thanks to spatial locality benefits within pages. Second, moving data always at a \emph{fixed} granularity (\textit{cache-line} via LLC or \textit{page} via \emph{local memory}) cannot provide robustness  %high system performance 
across heterogeneous applications and network configurations: some applications can benefit from cache line (e.g., \emph{pr}, \emph{nw}) or page granularity (e.g., \emph{pf}, \emph{dr}) data movements, while the best-performing granularity also depends on network characteristics (e.g., \emph{bf}, \emph{ts}). Third, \emph{naively} moving data at \emph{both} granularities (\textit{cache-line+page}) to serve
data requests with the latency of the packet that arrives earlier to the \computeComponent{} is still quite inefficient, while critical cache line requests are still queued behind large concurrently accessed pages. \revised{In contrast, Figure~\ref{fig:motivation-exab} shows that \myName{} (see §\ref{KeyIdeasbl}) significantly reduces data movement overheads in \disaggrSystems{} across various network/application characteristics.}
%\revised{Instead, Fig.~\ref{fig:motivation-exab} shows that \myName{} significantly improves system performance and data movement costs for various network and application characteristics.}
%Instead, \myName{} intelligently selects between two data movement granularities and significantly alleviates data movement overheads in \disaggrSystems{}, while providing low cost page migration, software transparency and robustness.

%To this end, we design \myName{} to significantly alleviate data movement costs in \disaggrSystems{}, and provide low overhead page migration, software transparency and robustness to variations in network, architecture and application characteristics.


\vspace{-1pt}
\section{Prior Work}
%\noindent\textbf{\large{2. Prior State-of-the-Art Works}}

Prior works~\cite{Shan2018LegoOS,Angel2020Disaggregation,Nitu2018Zombieland,Han2013Network,Calciu2021Rethinking,Aguilera2017Remote,Zhang2020RethinkingDM,Lim2012System,Chenxi2020Semeru,Pengfei2021OneSided,Bindschaedler2020Hailstorm,Peng2020Underutilization,Lagar2019Software,Gu2017Infiniswap,Aguilera2018Remote, Lee2021MIND,Pinto2020ThymesisFlow,Katrinis2016dredbox,guo2021clio,Buragohain2017DiME,Gao2016Network,Rao2016IsMemory,Zervas2018Optically,Gouk2022Direct,Zhou2022Carbink} propose OS kernels, system-level solutions, software management systems, architectures for \disaggrSystems{}. These works do not tackle the data movement challenge in \disaggrSystems{}, and thus our work is orthogonal to them.


Prior works on hybrid systems~\cite{Dong2010Simple,Liu2017Hardware,Jiang2010CHOP,Kotra2018Chameleon,Prodromou2017MemPod,Agarwal2017Thermostat,Mitesh2015Heterogeneous,Kai2017Unimem,Loh2011Efficiently,Loh2012Supporting,Chou2014Cameo,Ryoo2017Silcfm,Jevdjic2013Footprint} integrate die-stacked DRAM~\cite{HBM} as DRAM cache of a large main memory~\cite{Agarwal2017Thermostat,Dong2010Simple,Jiang2010CHOP} in a monolithic server, and tackle high page movement costs in two-tiered physical memory via page placement/hot page selection schemes or by moving data at smaller granularity, e.g., cache line. However, data movement in \disaggrSystems{} poses fundamentally different challenges.\cgiannou{not addressed in prior works} First, accesses across the network are significantly slower than within the server, thus intelligent page placement/movement cannot by itself address these high costs. Second, \disaggrSystems{} incur significant variations in access latencies %and bandwidth 
based on the current network architecture and concurrent jobs sharing the \memoryComponents{}/network, thus necessitating an solution primarily designed for robustness to this variability. Finally, \disaggrSystems{} \revised{include} independently managed \memoryComponents{} and networks \revised{shared by independent \computeComponents{} running unknown jobs.} Thus, unlike hybrid systems, the solution cannot \revised{assume that the memory management at the \memoryComponents{} can be fully controlled by the CPU side. Our work is the first to examine the data movement problem in fully \disaggrSystems{}, and design an effective solution for \disaggrSystems{}.}
%Finally, \disaggrSystems{} assume independently managed \memoryComponents{} and networks, shared with other unknown servers. Thus, unlike many hybrid systems, the solution cannot assume holistic control of both memory and host.
%Finally, \disaggrSystems{} \revised{include} independently managed \memoryComponents{} and networks, shared with \revised{many unknown jobs}. Thus, unlike hybrid systems, the solution cannot \revised{assume that the memory management is exclusively handled and controlled by the server side. Our work is the first to examine the data movement problem in fully \disaggrSystems{}, and design an effective disaggregated solution for such systems.}


%\cgiannou{1. Can we move the first argument as the last one? (seems to be the weaker between the three). 2. Fix writing in the 3rd argument}
%\cgiannou{Finally, \disaggrSystems{} include independently managed \memoryComponents{}, and memory management is distributed across \memoryComponents{}/network. Thus, the solution cannot assume a tight integration of the compute, memory and OS modules, while it need to also be \emph{disaggregated}. }

\section{\myName{}'s Key Ideas}\label{KeyIdeasbl}
%\noindent\textbf{\large{3. \myName{}'s Key Ideas}}

%\myName{} (Fig.~\ref{fig:daemon-design-exab}) is a software-transparent mechanism to alleviate data costs in \disaggrSystems{}, \revised{consisting} of three techniques.

\myName{} (Figure~\ref{fig:daemon-design-exab}) is an adaptive and scalable mechanism to alleviate data costs in \disaggrSystems{}, \revised{consisting} of three techniques. 


\begin{figure}[h]
    \vspace{-8pt}
    \centering
    \includegraphics[width=\linewidth]{DaeMon_Overview2.pdf}
    \vspace{-16pt}
    \caption{High-level overview of \myName{}.}
    \label{fig:daemon-design-exab}
    \vspace{-2pt}
\end{figure}



\noindent\textbf{(I) Decoupled Multiple Granularity Data Movement.}  We integrate two separate hardware queues to serve data requests from \emph{remote memory} at two granularities, i.e., cache line (via the \emph{sub-block queue} to LLC) and page (via the \emph{page queue} to \emph{local memory}) granularity, and effectively \textit{prioritize} moving cache lines over moving pages via a \emph{bandwidth partitioning} approach: a queue controller serves cache line requests with a higher \emph{predefined fixed rate} than page requests to ensure that any given time a certain fraction of the bandwidth resources is always allocated to serve cache line moves fast.
%there are enough bandwidth resources to move critical cache lines fast. 
This key technique enables (i) low metadata overheads by retaining page migrations, (ii) high performance by leveraging data locality within pages, and (iii) fewer slowdowns in cache line data movements that are on the critical path, from expensive page moves that may have been previously triggered.



\noindent\textbf{(II) Selection Granularity Data Movement.} To provide an adaptive data movement solution, we include in each \computeComponent{} two separate hardware buffers to track pending data migrations for both cache line (via the \emph{inflight sub-block buffer}) and page (via the \emph{inflight page buffer}) granularity, and a selection granularity unit to decide if a data request should be served by cache line, page or \emph{both} based on the utilization of the \emph{inflight} buffers. Given that \myName{} prioritizes cache line over page moves, the inflight buffers are utilized in different ways, allowing us to capture the application behavior and the system load during runtime. For example:
 (a) If there is \emph{low locality} within pages, the page buffer has higher utilization than the sub-block buffer (cache lines are prioritized), thus the selection unit favors moving cache lines and throttles pages (and vice-versa). 
(b) Under low \emph{bandwidth utilization} scenarios, the page buffer utilization is low, thus the selection unit schedules more page movements (or both granularities) to obtain data locality benefits (and vice-versa). 


\noindent\textbf{(III) Link Compression on Page Movements.} We employ hardware compression units at both the \computeComponents{} and \memoryComponents{} to highly compress pages migrated over the network. \emph{Link compression} on page moves reduces the network bandwidth consumption and alleviates network bottlenecks.




\noindent\textbf{Synergy of Three Techniques.} 
%Neither technique is independently effective under all network/application characteristics. Thus, 
\myName{} cooperatively integrates all three techniques to significantly alleviate data movement overheads, and provide robustness towards network, architecture and application characteristics: \\
(1) Prioritizing requested cache lines helps \myName{} to tolerate high (de)compression latencies in page migrations over the network, while also leveraging benefits of page migrations (low metadata costs, spatial locality in pages). \\
(2) Compressed pages consume less network bandwidth, enabling \myName{} to reserve part of the bandwidth to effectively prioritize critical path cache line accesses. \\
(3) Compression on page moves helps \myName{} to adapt to the data compressibility: if the pages are highly compressible, the inflight page buffer empties at a faster rate, and \myName{} favors sending more pages (and vice-versa).
%(3) Using link compression to transfer pages helps \myName{} adapt to the application data compressibility: if the pages are highly compressible, the inflight page buffer empties at a faster rate, and \myName{} favors sending more pages (and vice-versa).



\section{\myName{}'s Key Results}
%\noindent\textbf{\large{4. \myName{}'s Contributions}}

We extend Sniper~\cite{carlson2011etloafsaapms} to simulate \disaggrSystems{}, and evaluate capacity intensive workloads from graph processing, HPC, data analytics, bioinformatics, machine learning domains. \myName{} reduces data access costs and improves performance by 3.06$\times$ and 2.39$\times$, respectively, over the widely-adopted approach of moving data at a page granularity. \myName{} leverages the synergy of all three techniques to provide robustness, while retaining the spatial locality, transparency and metadata management benefits of page granularity movements. We show that \myName{} achieves high system performance for various network/architecture configurations and applications (Figure~\ref{fig:multi-exab} top), and multiple concurrently running jobs in the \disaggrSystem{} (Figure~\ref{fig:multi-exab} bottom), compared to the widely-adopted approach of moving data at page granularity.




\begin{figure}[h]
    \vspace{-2pt}
    \centering
    \includegraphics[width=\linewidth]{multimem_exab.pdf}
    \includegraphics[width=\linewidth]{multibench_speedup_netlat_100_bwsf_2_exab.pdf}
    \vspace{-12pt}
    \caption{\myName{}'s benefits over the \emph{page} scheme, (i) varying the \memoryComponents{}, network bandwidth and application, and (ii) running multiple applications in a 4-CPU \computeComponent{} and a \memoryComponent{}.}
    \label{fig:multi-exab}
    %\vspace{-14pt}
\end{figure}







%\section{Why ASPLOS}
%\noindent\textbf{\large{Why ASPLOS?}}
%\disaggrSystems{} require redesigning all levels of the computing stack. Our work tackles data movement, an important system challenge to be addressed in order to fully leverage the benefits of resource disaggregation.


